Preliminary clustering properties of the DESI BGS bright targets using DR9 Legacy Imaging Surveys

We characterise the selection cuts and clustering properties of a magnitude-limited sample of bright galaxies that is part of the Bright Galaxy Survey (BGS) of the Dark Energy Spectroscopic Instrument (DESI) using the ninth data release of the Legacy Imaging Surveys (DR9). We describe changes in the DR9 selection compared to the DR8 one as explored in Ruiz-Macias et al. (2021). We also compare the DR9 selection in three distinct regions: BASS/MzLS in the north Galactic Cap (NGC), DECaLS in the NGC, and DECaLS in the south Galactic Cap (SGC). We investigate the systematics associated with the selection and assess its completeness by matching the BGS targets with the Galaxy and Mass Assembly (GAMA) survey. We measure the angular clustering for the overall bright sample (r $\leq$ 19.5) and as function of apparent magnitude and colour. This enables to determine the clustering strength and slope by fitting a power-law model that can be used to generate accurate mock catalogues for this tracer. We use a counts-in-cells technique to explore higher-order statistics and cross-correlations with external spectroscopic data sets in order to check the evolution of the clustering with redshift and the redshift distribution of the BGS targets using clustering-redshifts. While this work validates the properties of the BGS bright targets, the final target selection pipeline and clustering properties of the entire DESI BGS will be fully characterised and validated with the spectroscopic data of Survey Validation.

==> syst.tex <==
\section{Study of potential systematics}
\label{sec:syst}

In this section we investigate the potential systematics associated with the BGS target selection. Fig.~\ref{fig:syst} shows the variation of the BGS target density with common imaging systematics for BASS/MzLS (in blue), DECaLS-NGC (in red) and DECaLS-SGC (in green). We can see that the strongest dependence is due to the stars with a maximum  7 per cent variation in the target density with stellar density, which was also found with DR8 DECaLS~\citep{Ruiz+21}. Only {\it Gaia} stars with $12 < G < 17$ are used here, and we remind the reader that only the brightest stars with $G < 13$ are masked (recall that $G$ is the {\it Gaia} $G$-band magnitude). In Section~\ref{sec:xstars}, we study the cross-correlation signal of the BGS targets with this stellar catalogue. We also check the behaviour of the BGS targets in the vicinity of the large galaxies (Section~\ref{sec:xLG}) to see whether additional cuts are necessary to remove spurious objects. Then we validate the target selection and the additional cuts that define a cleaner catalogue for clustering analysis by comparing with GAMA in Section~\ref{sec:check}. Both Sections~\ref{sec:xstars} and~\ref{sec:xLG} use auto-correlation and cross-correlation functions that are determined using the Landy-Szalay estimator~\citep{LandySzalay93} defined by equation~\ref{eq:LS} in Section~\ref{sec:ang-corr}.

 \begin{figure*}
	\centering
	\includegraphics[scale=0.4]{Figures/systematics_bgs_bright.png}
    %\vskip -0.2cm
    \caption{\BGSB~ target density variation with imaging systematics for BASS/MzLS (red), DECaLS-NGC (green) and DECaLS-SGC (blue).}
    \label{fig:syst} 
\end{figure*}

%Update figure for DR9 no LG new fracs with BASS/MzlS in blue, DECaLS-NGC in red and DECaLS-SGC in green.}
%-----------------------------
%-----------------------------

\subsection{Cross-correlation with stars}
\label{sec:xstars}



%-----------------------------
%-----------------------------

\subsection{Cross-correlation with large galaxies}
\label{sec:xLG}


%-----------------------------
%-----------------------------








